QuPeD: Quantized Personalization via Distillation with Applications to Federated Learning

Traditionally, federated learning (FL) aims to train a single global model while collaboratively using multiple clients and a server. Two natural challenges that FL algorithms face are heterogeneity in data across clients and collaboration of clients with {\em diverse resources}. In this work, we introduce a \textit{quantized} and \textit{personalized} FL algorithm QuPeD that facilitates collective (personalized model compression) training via \textit{knowledge distillation} (KD) among clients who have access to heterogeneous data and resources. For personalization, we allow clients to learn \textit{compressed personalized models} with different quantization parameters and model dimensions/structures. Towards this, first we propose an algorithm for learning quantized models through a relaxed optimization problem, where quantization values are also optimized over. When each client participating in the (federated) learning process has different requirements for the compressed model (both in model dimension and precision), we formulate a compressed personalization framework by introducing knowledge distillation loss for local client objectives collaborating through a global model. We develop an alternating proximal gradient update for solving this compressed personalization problem, and analyze its convergence properties. Numerically, we validate that QuPeD outperforms competing personalized FL methods, FedAvg, and local training of clients in various heterogeneous settings.

==> introduction.tex <==


Federated Learning (FL) is a learning procedure where the aim is to utilize vast amount of data residing in numerous (in millions) edge devices (clients) to train machine learning models without collecting clients' data \citep{mcmahan2017communicationefficient}. Formally, if there are $n$ clients and $f_i$ denotes the local loss function at client $i$, then traditional FL learns a single global model by minimizing % the following objective: % function: 
\begin{align} \label{fed1}
	\argmin_{\bw\in\R^d} \Big(f(\bw) := \frac{1}{n} \sum_{i=1}^n f_i(\bw)\Big).
\end{align}
It has been realized lately that a {\em single} model may not provide good performance to all the clients in settings where data is distributed {\em heterogeneously}.
This leads to the need for personalized learning, where each client wants to learn its own model  \citep{fallah2020personalized,dinh2020personalized}. Since each client may not have sufficient data to learn a generalizable model, in personalized FL process, clients maintain personalized models locally and utilize other clients' data via a global model\footnote{This is a particular form of co-ordination where a global model $\wbf$ facilitates the co-ordination among multiple local models.}.
%
{\em Resource diversity} among clients, which is inherent to FL as the participating edge devices may vary widely in terms of resources, is often overlooked in personalized FL works. In FL scenarios, model compression can become critical as it would let devices with different resource constraints utilize complex models.

In this work, we propose a model compression framework\footnote{Model compression is a process that allows inference time deployment of a model while compressing its size. Though model compression is a general term comprising different methods, we will focus on the quantization aspect of it.} for personalized FL via knowledge distillation (KD) \citep{hinton2015distilling} that addresses the both aforementioned types of heterogeneity (in data and resources) in a unified manner. 
For the first time in literature our framework allows collaboration among clients, that have different resource requirements in terms of {\em precision} and {\em model dimension/structure}, for learning personalized quantized models (PQMs). Our goal is to obtain compressed models for inference time when the clients are restricted to less amount of resources and models are frequently used. %\footnote{Assuming more resources are available for training and not for inference time is highly practical in FL with edge devices ({\em e.g.}, smartphones), where model training is typically done when the phone is charging and is idle (so more power/memory is available), whereas, inference is more frequent and is done when phones are actively used and have other functions. Since relatively less power/memory is available during inference time, the deployed model should respect stricter resource constraints.}.
To achieve this goal in an efficient way, we learn the compression parameters for each client by including quantization levels in the optimization problem itself.
First, we investigate our approach in the {\em centralized} setup, by formulating a relaxed optimization problem and minimizing that through alternating proximal gradient steps, inspired by \cite{Bolte13}.
%
To extend this to a distributed setup, we employ our centralized model quantization algorithm locally at clients and introduce KD loss for collaboration of personalized and global models. Although there have been works where KD is used in personalized FL \citep{li2019fedmd}, we, for the first time, formalize it as an optimization problem and analyze the convergence properties. Moreover, as far as we are aware, this is the first work that considers learning PQMs with potentially different dimensions/structures FL.

\textbf{Contributions.}
Our contributions are as follows: %\\\vspace{-0.55cm}
\begin{itemize}[leftmargin=*,topsep=0pt,nosep]
	\item We propose a novel relaxed optimization problem that enables optimization over quantization values (centers) as well as the model parameters. We use alternating proximal updates to minimize the objective and analyze its convergence properties.  %\\\vspace{-0.55cm}
%Although the training is in full precision, in the end of training we arrive at a model that can be compressed without significant loss. \\\vspace{-0.55cm}

\item More importantly, we for the first time state a personalized FL optimization problem where clients can have different model dimensions and precision. To optimize this problem we propose an algorithm that combines alternating proximal gradient updates with knowledge distillation.  %\\\vspace{-0.55cm}

\item  In centralized setup we recover the convergence rate of $\mathcal{O}(\frac{1}{T})$ in \cite{Bolte13}. We observe that aggressiveness of quantization has a scaling effect on the convergence rate. In federated setting the convergence result includes an error term that depends on the heterogeneity in data \footnote{This is commonly observed in FL algorithms with heterogeneous data assumptions \cite{fallah2020personalized,dinh2020personalized}.}. \cred{ Furthermore, we observe that convergence rate depends on a smoothness term characterizing the average smoothness of the models across all clients.}

\item  We perform image classification experiments on 3 datasets in various resource and data heterogeneity settings. We compare QuPeD to Per-FedAvg \citep{fallah2020personalized}, pFedMe \citep{dinh2020personalized}, FedAvg \citep{mcmahan2017communicationefficient} and local training of clients in terms of classification accuracy. \cred{We observe that QuPeD outperforms all these methods.} 
\end{itemize}
Our work should not be confused with works in distributed/federated learning, where models/gradients are compressed for {\em communication efficiency} \citep{basu2019qsparse,karimireddy2019error}. The main goal of this work is to obtain quantized personalized models for inference, that are suited for each client's resources. Although it is our not main goal, we still achieve communication efficiency through local iterations.


%\subsection{Related Work} 
\textbf{Related work.} To the best of our knowledge, this is the first work in personalized federated learning where the aim is to learn quantized and personalized models potentially having different dimensions/structures for inference. Our work can be seen in the intersection of {\em personalized federated learning} and {\em learning quantized models}, we also employ {\em knowledge distillation} for collaboration.

\iffalse
\textit{Personalized federated learning.}
As mentioned before, personalized FL is used in heterogeneous scenarios when a single global model falls short for the learning task. % In such cases, each client would locally retain a personalized model throughout the training phase and collaborate with other clients through a global model. 
Recent work adopted different approaches for learning personalized models: 
{\sf(i)} Combine global and local models throughout the training \cite{deng2020adaptive,mansour2020approaches,hanzely2020federated};
{\sf (ii)} first learn a global model and then personalize it locally by updating it using clients' local data \cite{fallah2020personalized}; 
{\sf (iii)} consider multiple global models to collaborate among only those clients that share similar personalized models \cite{zhang2021personalized}; and
{\sf (iv)} augment the traditional FL  objective via a penalty term that enables collaboration between global and personalized models \cite{hanzely2020federated,hanzely2020lower,dinh2020personalized}.
\fi
\textit{Personalized federated learning.}
As mentioned before, personalized FL is used in heterogeneous scenarios when a single global model falls short for the learning task.
Recent work adopted different approaches for learning personalized models: 
{\sf(i)} Combine global and local models throughout the training \citep{deng2020adaptive,mansour2020approaches,hanzely2020federated};
{\sf (ii)} first learn a global model and then personalize it locally by updating it using clients' local data \citep{fallah2020personalized}; 
{\sf (iii)} consider multiple global models to collaborate among only those clients that share similar personalized models \citep{zhang2021personalized,mansour2020approaches,ghosh2020efficient,smith2017federated}; 
{\sf (iv)} augment the traditional FL  objective via a penalty term that enables collaboration between global and personalized models \citep{hanzely2020federated,hanzely2020lower,dinh2020personalized}; and
{\sf (v)} distillation of global model to personalized local models \citep{lin2020ensemble}. 

%\cblue{In an another approach of clustered FL \cite{sattler2019clustered}, clients with similar data distributions collaborate to learn personalized models \citep{mansour2020approaches}.}
%This collaboration can be in different ways. One way is through combining the global and local model parameters to obtain individual personalized models \cite{deng2020adaptive,mansour2020approaches,hanzely2020federated}. 
%Zhang et al.~\cite{zhang2021personalized} considered multiple global models to collaborate among only the clients that share similar personalized models. Fallah et al.~\cite{fallah2020personalized} aimed to find personalized models for heterogeneous clients through performing few updates on clients' local data after learning the common model. %; they studied this problem in the Model-Agnostic Meta-Learning framework \cite{Finn_maml17}. 
%In \cite{hanzely2020federated,hanzely2020lower,dinh2020personalized}, authors augment the traditional FL  objective via a penalty term that enables collaboration between global and personalized models.
%\TODO{Not clear: In Clustered Federated Learning \cite{sattler2019clustered} approaches allow clients with similar data distributions to collaborate \citep{mansour2020approaches}.}

\textit{Learning quantized models.}
Training quantized neural networks has been a topic of great interest in the last few years, and extensive research resulted in training quantized networks with precision of as low as 1-bit without significant loss in performance; see \citep{Bin_survey,comprehensive_survey} for surveys.
%\cred{ There are two main approaches in obtaining quantized models. Firstly, one can simply train a model and then do a post-training quantization that is agnostic to training procedure; see for example \citep{BannerNS19}. The downside of doing a post-training quantization is that the loss minimization problem for quantization is not related to the empirical loss function. Consequently, there is no guarantee that one will obtain a compressed model that has good performance. As opposed to post-training quantization, the aim of learning quantized models is to learn the quantization itself during the training \citep{courbariaux2016binarized,courbariaux2015binaryconnect}.} 
There are two kinds of approaches for training quantized networks that are of our interest. The first approximates the hard quantization function by using a soft surrogate \citep{Yang_2019_CVPR, gong2019differentiable}, while the other one iteratively projects the model parameters onto the fixed set of centers \citep{bai2018proxquant,BinaryRelax}. Each approach has its own limitations; see Section~\ref{sec:problem} for a discussion. While the initial focus in learning quantized networks was mainly on achieving good empirical performance, there exist some works that analyzed convergence properties. \cite{li2017training} gave the first convergence guarantees by analyzing the algorithm proposed in \citep{courbariaux2015binaryconnect} using convexity assumptions. % and proposing a stochastic rounding scheme which resulted in a better convergence guarantee. 
Later, \cite{BinaryRelax} showed convergence results for non-convex functions but under an orthogonality assumption between the quantized and unquantized weights. More recently, \cite{bai2018proxquant} gave a convergence result for a relaxed/regularized loss function using proximal gradient updates. Note that all of the above works were done in centralized setting.

\textit{Knowledge distillation.} Knowledge distillation \citep{hinton2015distilling} is a successful framework in transfer learning that is generally used to train a small student network using the soft labels generated by a deep teacher network. It can also be used to train two or more networks mutually by switching teacher and students in each iteration \citep{zhang2018deep}. KD has been employed in FL settings as an alternative to simple aggregation which is not feasible when clients have models with different dimensions \citep{LinKSJ20}. In \citep{li2019fedmd} authors used KD in personalized FL by assuming existence of a public dataset and in \citep{shen2020federated} authors integrated Deep Mutual Learning \citep{zhang2018deep} for personalized FL. However, none of the previous works formalized an optimization problem and analyzed convergence properties. Furthermore, for the first time our method uses reverse KL updates to train the global model and allows clients to train models with different precision and different dimension through local alternating proximal updates. In \citep{polino2018model}, authors use KD in combination with quantization in a centralized case for model compression; in contrast, we don't use KD for model compression but use in collaboration of personalized and global models.


\iffalse
There have been mainly two approaches for training quantized networks. The first one is where we keep the model parameters $\bx$ quantized throughout the training by replacing the objective function $f(\bx)$ with $f(Q_{\calC}(\bx))$ for a {\em fixed} set $\calC$ of centers, where $Q$ is a hard quantization function. Due to the staircase nature of $Q$ (which makes its derivative equal to $0$ almost everywhere), Yang et al.~\cite{Yang_2019_CVPR} and Cheng et al.~\cite{cheng2018differentiable} proposed differentiable soft quantization functions, which would enable training of DNN's in the presence of a quantization-like operation.
In an another approach, we take explicit we modify the objective by augmenting it with a regularizer

There have been mainly two approaches for training quantized networks with a {\em fixed} set of centers. The first one keeps the model parameters quantized throughout the training phase, while the other one explicitly projects the model parameters onto the fixed set of centers. Due to the limitations of the Since the quantization function in the first approach is a staircase function

One of the main challenges in training quantized networks is the fact that quantization is a staircase function for which the derivative is 0 almost everywhere. To cope with this, Yang et al.~\cite{Yang_2019_CVPR} and Cheng et al.~\cite{cheng2018differentiable} proposed differentiable soft quantization functions, which would enable training of DNN's in the presence of a quantization-like operation. Another way to learn quantized models is to modify the loss function. Bai et al.~\cite{bai2018proxquant} and Yin et al.~\cite{BinaryRelax} augment the loss function through a regularizer that helps weights to be trained such that quantization does not result in significant degradation. 
\fi


\textbf{Paper organization.} In Section~\ref{sec:problem} we formulate the optimization problem to be minimized. In Sections~\ref{sec:centralized} and~\ref{sec:personalized}, we describe our algorithms along-with the main convergence results for the centralized and personalized settings, respectively, and give a proof outline in Section~\ref{sec:proof_outlines}. Section~\ref{sec:experiments} provides numerical results. Omitted proofs/details are in appendices, provided as part of the supplementary material.



==> introduction_DD_saved.tex <==


Federated Learning (FL) is a learning procedure where the aim is to utilize vast amount of data residing in numerous (in millions) edge devices (clients) to train machine learning models without collecting clients' data \citep{mcmahan2017communicationefficient}. Formally, if there are $n$ clients and $f_i$ denotes the local loss function at client $i$, then traditional FL learns a single global model by minimizing % the following objective: % function: 
\begin{align} \label{fed1}
	\argmin_{\bw\in\R^d} \Big(f(\bw) := \frac{1}{n} \sum_{i=1}^n f_i(\bw)\Big).
\end{align}
It has been realized lately that a {\em single} model may not provide good performance to all the clients in settings where data is distributed {\em heterogeneously}.
This leads to the need for personalized learning, where each client wants to learn its own model  \citep{fallah2020personalized,dinh2020personalized}. Since a locally learned client model may not generalize well due to insufficient data, in personalized FL process, clients maintain personalized models locally and utilize other clients' data via a global model.
%
{\em Resource diversity} among clients, which is inherent to FL as the participating edge devices may vary widely in terms of resources, is often overlooked in personalized FL literature. This resource diversity may necessitate clients to learn personalized models with {\em different precision} as well as {\em different dimension/architecture}. Systematically studying both these resource heterogeneity together with data heterogeneity in personalized FL is the primary objective of this paper. 
%In FL scenarios, model compression can become critical as it would let devices with different resource constraints utilize complex models.

In this work, we propose a model compression framework\footnote{Model compression (MC) allows inference time deployment of a compressed model. Though MC is a generic term comprising different methods, we will focus on its quantization (number of bits per model parameter) aspect.} for personalized FL via knowledge distillation (KD) \citep{hinton2015distilling} that addresses both data and resource heterogeneity in a unified manner. Our framework allows collaboration among clients with different resource requirements both in terms of {\em precision} as well as {\em model dimension/structure}, for learning personalized quantized models (PQMs). 
Motivated by FL, where edge devices are resource constrained when actively used ({\em e.g.} when several applications are actively running on a battery powered smartphone) and available for training when not in use ({\em e.g.}, while charging and on wi-fi), we do training in full precision for learning compressed models to be deployed for {\em inference time}.
%Our goal is to obtain compressed models for {\em inference time} when the clients are resource constrained and models are frequently used ({\em e.g.}, using smartphones in the daytime), and our training is in full precision ({\em e.g.}, training using smartphones while charging in the night).
%\footnote{Assuming more resources are available for training and not for inference time is highly practical in FL with edge devices ({\em e.g.}, smartphones), where model training is typically done when the phone is charging and is idle (so more power/memory is available), whereas, inference is more frequent and is done when phones are actively used and have other functions. Since relatively less power/memory is available during inference time, the deployed model should respect stricter resource constraints.}.
For efficient model compression, we learn the quantization parameters for each client by including quantization levels in the optimization problem itself.
First, we investigate our approach in a {\em centralized} setup, by formulating a relaxed optimization problem and minimizing it through alternating proximal gradient steps, inspired by \cite{Bolte13}.
%
To extend this to FL for learning PQMs with {\em different} dimensions/architectures, we employ our centralized algorithm locally at clients and introduce KD loss for collaboration of personalized and global models. Although there exist empirical works where KD is used in personalized FL \citep{li2019fedmd}, we formalize it as an optimization problem, solve it using alternating proximal updates, and analyze its convergence. 
%As far as we are aware, this is the first work that considers learning PQMs with potentially different dimensions/structures.

\textbf{Contributions.}
Our contributions can be summarized as follows: \vspace{-0.2cm}
\begin{itemize}[leftmargin=*,topsep=0pt,nosep]
	\item In the centralized case, we propose a novel relaxed optimization problem that enables optimization over quantization values (centers) as well as model parameters. We use alternating proximal updates to minimize the objective and analyze its convergence properties.  %\\\vspace{-0.55cm}
%	 We use alternating proximal updates to minimize the objective and analyze its convergence properties.  %\\\vspace{-0.55cm}

	
	\item More importantly, our work is the first to formulate a personalized FL optimization problem where clients may have different model dimensions and precision requirements for their personalized models. 
	Our proposed scheme combines alternating proximal updates with knowledge distillation.
%	To optimize this problem we propose an algorithm that combines alternating proximal gradient updates with knowledge distillation.  %\\\vspace{-0.55cm}
	
	\item For optimizing a non-convex objective, in the centralized setup, we recover the standard convergence rate of $\calO(\nicefrac{1}{T})$ % from \cite{Bolte13}, 
	(despite optimizing over quantization centers), and for federated setting, we recover the standard convergence rate of $\calO(\nicefrac{1}{\sqrt{T}})$ % from \citep{dinh2020personalized}, 
	(despite learning PQMs with different precisions/dimensions). 
	%We observe that aggressiveness of quantization has a scaling effect on the convergence rate. 
	%In the federated setting, our convergence bound has an error term that depends on the heterogeneity in data;\footnote{This is commonly observed in FL algorithms with heterogeneous data \citep{fallah2020personalized,dinh2020personalized}.} furthermore, we observe that convergence rate depends on multiplication of two terms: one characterizing client's local model smoothness and the other data heterogeneity with respect to overall data distribution.
	In the federated setting, our convergence bound has an error term that depends on multiplication of two terms averaged over clients: one characterizing client's local model smoothness and the other data heterogeneity with respect to overall data distribution.\footnote{ An error term depending on data heterogeneity is commonly observed in personalized FL algorithms \citep{fallah2020personalized,dinh2020personalized}.}
	
	\item  We perform image classification experiments on multiple datasets in various resource and data heterogeneity settings. We compare performance of QuPeD to Per-FedAvg \citep{fallah2020personalized}, pFedMe \citep{dinh2020personalized}, FedAvg \citep{mcmahan2017communicationefficient} and local training of clients. %We observe that QuPeD outperforms competing methods. 
We observe that even with aggressive 2 bit quantization, QuPeD outperforms other {\em full-precision} personalized FL methods on the CIFAR-$10$ dataset.
\end{itemize}
Our work should not be confused with works in distributed/federated learning, where models/gradients are compressed for {\em communication efficiency} \citep{basu2019qsparse,karimireddy2019error}. We also achieve communication efficiency through local iterations, but the main goal of our work is personalized quantization for inference. % to obtain personalized quantized models for inference, that are suited for each client's resources. %Although it is our not main goal, we still achieve communication efficiency through local iterations.


%\subsection{Related Work} 
\textbf{Related work.} To the best of our knowledge, this is the first work in personalized federated learning where the aim is to learn quantized and personalized models potentially having different dimensions/structures for inference. Our work can be seen in the intersection of {\em personalized federated learning} and {\em learning quantized models}; we also employ {\em knowledge distillation} for collaboration.

\iffalse
\textit{Personalized federated learning:}
As mentioned before, personalized FL is used in heterogeneous scenarios when a single global model falls short for the learning task. % In such cases, each client would locally retain a personalized model throughout the training phase and collaborate with other clients through a global model. 
Recent work adopted different approaches for learning personalized models: 
{\sf(i)} Combine global and local models throughout the training \cite{deng2020adaptive,mansour2020approaches,hanzely2020federated};
{\sf (ii)} first learn a global model and then personalize it locally by updating it using clients' local data \cite{fallah2020personalized}; 
{\sf (iii)} consider multiple global models to collaborate among only those clients that share similar personalized models \cite{zhang2021personalized}; and
{\sf (iv)} augment the traditional FL  objective via a penalty term that enables collaboration between global and personalized models \cite{hanzely2020federated,hanzely2020lower,dinh2020personalized}.
\fi
\textit{Personalized federated learning:}
%As mentioned before, personalized FL is used in heterogeneous scenarios when a single global model falls short for the learning task.
Recent works adopted different approaches for learning personalized models: 
{\sf(i)} Combine global and local models throughout the training \citep{deng2020adaptive,mansour2020approaches,hanzely2020federated};
{\sf (ii)} first learn a global model and then personalize it locally \citep{fallah2020personalized}; 
{\sf (iii)} consider multiple global models to collaborate among only those clients that share similar personalized models \citep{zhang2021personalized,mansour2020approaches,ghosh2020efficient,smith2017federated}; 
{\sf (iv)} augment the traditional FL  objective via a penalty term that enables collaboration between global and personalized models \citep{hanzely2020federated,hanzely2020lower,dinh2020personalized}; and
{\sf (v)} distillation of global model to personalized local models \citep{lin2020ensemble}. 

%\cblue{In an another approach of clustered FL \cite{sattler2019clustered}, clients with similar data distributions collaborate to learn personalized models \citep{mansour2020approaches}.}
%This collaboration can be in different ways. One way is through combining the global and local model parameters to obtain individual personalized models \cite{deng2020adaptive,mansour2020approaches,hanzely2020federated}. 
%Zhang et al.~\cite{zhang2021personalized} considered multiple global models to collaborate among only the clients that share similar personalized models. Fallah et al.~\cite{fallah2020personalized} aimed to find personalized models for heterogeneous clients through performing few updates on clients' local data after learning the common model. %; they studied this problem in the Model-Agnostic Meta-Learning framework \cite{Finn_maml17}. 
%In \cite{hanzely2020federated,hanzely2020lower,dinh2020personalized}, authors augment the traditional FL  objective via a penalty term that enables collaboration between global and personalized models.
%\TODO{Not clear: In Clustered Federated Learning \cite{sattler2019clustered} approaches allow clients with similar data distributions to collaborate \citep{mansour2020approaches}.}

\textit{Learning quantized models:}
%Training quantized neural networks has been a topic of great interest in the last few years, and extensive research resulted in training quantized networks with precision of as low as 1-bit without significant loss in performance; see \citep{Bin_survey,comprehensive_survey} for surveys.
%\cred{ There are two main approaches in obtaining quantized models. Firstly, one can simply train a model and then do a post-training quantization that is agnostic to training procedure; see for example \citep{BannerNS19}. The downside of doing a post-training quantization is that the loss minimization problem for quantization is not related to the empirical loss function. Consequently, there is no guarantee that one will obtain a compressed model that has good performance. As opposed to post-training quantization, the aim of learning quantized models is to learn the quantization itself during the training \citep{courbariaux2016binarized,courbariaux2015binaryconnect}.} 
There are two kinds of approaches for training quantized networks that are of our interest. The first one approximates the hard quantization function by using a soft surrogate \citep{Yang_2019_CVPR, gong2019differentiable}, while the other one iteratively projects the model parameters onto the fixed set of centers \citep{bai2018proxquant,BinaryRelax}. Each approach has its own limitation; see Section~\ref{subsec:centralized-motivation} for a discussion. While the initial focus in learning quantized networks was on achieving good empirical performance, there are some works that analyzed convergence properties \citep{li2017training,BinaryRelax,bai2018proxquant}, but only in the centralized case. 
%\cite{li2017training} provided the first convergence guarantee by analyzing the algorithm proposed in \citep{courbariaux2015binaryconnect} using convexity assumptions. % and proposing a stochastic rounding scheme which resulted in a better convergence guarantee. 
%Later, \cite{BinaryRelax} showed convergence results for non-convex functions but under an orthogonality assumption between the quantized and unquantized weights. 
Among these, \cite{bai2018proxquant} analyzed convergence for a relaxed/regularized loss function using proximal updates.

\textit{Knowledge distillation (KD):} KD \citep{hinton2015distilling} is a framework for transfer learning that is generally used to train a small student network using the soft labels generated by a deep teacher network. It can also be used to train two or more networks mutually by switching teacher and students in each iteration \citep{zhang2018deep}. KD has been employed in FL settings as an alternative to simple aggregation which is not feasible when clients have models with different dimensions \citep{lin2020ensemble}. \cite{li2019fedmd} used KD in personalized FL by assuming existence of a public dataset.
%, \cred{and \cite{shen2020federated} extended framework of \citep{zhang2018deep} to personalized FL}.
\cite{polino2018model} used KD in combination with quantization in a centralized case for model compression; in contrast, we do not use KD for model compression but for collaboration between personalized and global model. Unlike the above works which are empirical, our paper is the first to formalize an optimization problem for personalized FL training with KD and analyze its convergence properties. Our proposed scheme yields personalized client models with different precision/dimension through local alternating proximal updates; see Section~\ref{subsec:KD-motivate} for details.    


%All these are empirical works and none of them formalized an optimization problem and analyzed convergence properties, like we do. In particular, we develop a method to train the global model from the local models and also to train local models with different precision/dimension through local alternating proximal updates; see Section~\ref{subsec:KD-motivate} for details.


\iffalse
There have been mainly two approaches for training quantized networks. The first one is where we keep the model parameters $\bx$ quantized throughout the training by replacing the objective function $f(\bx)$ with $f(Q_{\calC}(\bx))$ for a {\em fixed} set $\calC$ of centers, where $Q$ is a hard quantization function. Due to the staircase nature of $Q$ (which makes its derivative equal to $0$ almost everywhere), Yang et al.~\cite{Yang_2019_CVPR} and Cheng et al.~\cite{cheng2018differentiable} proposed differentiable soft quantization functions, which would enable training of DNN's in the presence of a quantization-like operation.
In an another approach, we take explicit we modify the objective by augmenting it with a regularizer

There have been mainly two approaches for training quantized networks with a {\em fixed} set of centers. The first one keeps the model parameters quantized throughout the training phase, while the other one explicitly projects the model parameters onto the fixed set of centers. Due to the limitations of the Since the quantization function in the first approach is a staircase function

One of the main challenges in training quantized networks is the fact that quantization is a staircase function for which the derivative is 0 almost everywhere. To cope with this, Yang et al.~\cite{Yang_2019_CVPR} and Cheng et al.~\cite{cheng2018differentiable} proposed differentiable soft quantization functions, which would enable training of DNN's in the presence of a quantization-like operation. Another way to learn quantized models is to modify the loss function. Bai et al.~\cite{bai2018proxquant} and Yin et al.~\cite{BinaryRelax} augment the loss function through a regularizer that helps weights to be trained such that quantization does not result in significant degradation. 
\fi
\textbf{Limitations.} For our convergence results stated in Theorems \ref{thm:centralized},\ref{thm:personalized}, we assume a uniform bound on gradients (assumption {\bf A.3, A.5}). Although this is a valid assumption for non-convex objectives considered in this paper, it is not satisfied for strongly-convex functions \cite{nguyen2019new}, hence our convergence analyses cannot be directly extended to that setting. We also acknowledge that there has been considerable interest in relaxing such an assumption for convergence analysis in FL \cite{haddadpour2021federated}; something we hope to achieve in a future work. Another technical limitation is the non-vanishing error term in Theorem~\ref{thm:personalized}, which is perhaps unavoidable due to data heterogeneity, and also appears in related works ({\em e.g.}, \cite{dinh2020personalized}). Lastly, a proper choice of tuning parameter $\lambda$ (see Section \ref{subsec:centralized-motivation}) is important for empirical performance of our algorithm. Understanding how to choose an appropriate value of $\lambda$ (and other parameters) is worth exploring.  We provide a detailed discussion about limitations in Appendix~\ref{appendix:Preliminaries}.

\textbf{Paper organization:} In Section~\ref{sec:problem}, we formulate the optimization problem to be minimized. In Sections~\ref{sec:centralized} and~\ref{sec:personalized}, we describe our algorithms along-with the main convergence results for the centralized and personalized settings, respectively. Section~\ref{sec:experiments} provides extensive numerical results. Omitted proofs/details are in appendices, provided as a part of the supplementary material.



